Fed-PISA: Federated Voice Cloning via Personalized Identity-Style Adaptation

Voice cloning for Text-to-Speech (TTS) aims to generate expressive and personalized speech from text using limited data from a target speaker. Federated Learning (FL) offers a collaborative and privacy-preserving framework for this task, but existing approaches suffer from high communication costs and tend to suppress stylistic heterogeneity, resulting in insufficient personalization. To address these issues, we propose Fed-PISA, which stands for Federated Personalized Identity-Style Adaptation. To minimize communication costs, Fed-PISA introduces a disentangled Low-Rank Adaptation (LoRA) mechanism: the speaker's timbre is retained locally through a private ID-LoRA, while only a lightweight style-LoRA is transmitted to the server, thereby minimizing parameter exchange. To harness heterogeneity, our aggregation method, inspired by collaborative filtering, is introduced to create custom models for each client by learning from stylistically similar peers. Experiments show that Fed-PISA improves style expressivity, naturalness, and speaker similarity, outperforming standard federated baselines with minimal communication costs.

==> intro.tex <==
\section{Introduction}
Modern Text-to-Speech (TTS) systems~\cite{wang2025spark, du2025cosyvoice, le2023voicebox} increasingly leverage voice cloning—the task of synthesizing speech in a target speaker's voice from arbitrary text inputs— to enable deep personalization: the synthesis of speech that captures not only a target speaker's vocal timbre but also their unique prosodic patterns and expressive style. The technical pursuit of this nuanced personalization has motivated the emergence of distinct research paradigms.

Among these, two main directions have emerged: high-fidelity zero-shot personalization based on style vectors or large-scale corpus~\cite{du2025cosyvoice, le2023voicebox, meng2025ds, chen2024emoknob}, along with lightweight on-device deployment via model compression and Parameter-Efficient Fine-Tuning (PEFT)~\cite{huang2023personalized, comini2025lightweight, bondaruk2025lorp, kwon2025parameter, fujita2024lightweight}. 
% While these methods advance speaker similarity and efficiency, 
Despite improvements in speaker similarity and efficiency, these methods share a fundamental limitation: the personalization process is isolated. 
This isolation creates ``style silos'', where a client's model is constrained by their own limited data, unable to leverage the rich stylistic heterogeneity present across a wider community of peers. 
Consequently, there is an increasing need for collaborative style learning across different clients under strict preservation of the local data privacy.

Under such circumstances, Federated Learning (FL)~\cite{zhang2021survey} offers a privacy-preserving approach that allows multiple clients to collaboratively train a model while keeping their private data on local devices. Existing FL-based TTS frameworks, such as FedSpeech~\cite{jiang2021fedspeech} and Federated Dynamic Transformer~\cite{hong2021federated}, primarily focus on backbone modification or partitioning to balance speaker-specific personalization with shared global knowledge. Nevertheless, training personalized TTS systems in this manner faces two key challenges. First, these methods often incur substantial computational and communication costs due to complex backbone modifications or large-scale parameter exchanges, hindering their deployment on resource-constrained edge devices. Second, they suppress the severe \textit{stylistic heterogeneity} exhibited in speech data distribution (e.g., variations in emotion, prosody) to preserve individual speaker timbre. FedSpeech isolates style features locally by parameter masking, while Federated Dynamic Transformer retains personalized layers that capture styles locally, aggregating only the general model. Such suppression limits the model from effectively learn diverse and expressive styles across heterogeneous client data, leading to insufficient model personalization capabilities. This motivates the exploration: 
\emph{\textbf{Can a federated TTS system effectively learn and utilize \textit{heterogeneous styles} across clients while maintaining low communication costs?}}
% \emph{\textbf{How can federated TTS systems be trained efficiently while leveraging {stylistic heterogeneity} as a resource for personalization rather than a challenge}}?

To tackle the aforementioned issues, we propose an efficient and personalized federated TTS framework, namely \textbf{Fed}erated \textbf{P}ersonalized \textbf{I}dentity-\textbf{S}tyle \textbf{A}daptation~(\textsc{Fed-PISA}). 
\textsc{Fed-PISA} builds upon the PEFT techniques, specifically inspired by recent studies that utilize Low-Rank Adaptation (LoRA) for single-client TTS personalization~\cite{bondaruk2025lorp, kwon2025parameter, fujita2024lightweight}.
It adapts the LoRA to a more complex federated setting and consists of two key components: 
(i) To improve efficiency and preserve speaker timbre, a decoupled LoRA mechanism is introduced. A private ID-LoRA is trained for each client and locally frozen to capture their unique speaker timbre robustly. A lightweight style-LoRA is used for communication on the server, effectively reducing costs. (ii) To leverage stylistic heterogeneity, we introduce a personalized aggregation strategy. Inspired by collaborative filtering in recommendation systems~\cite{isinkaye2015recommendation}, this strategy creates a custom-aggregated style model for each client by prioritizing updates from stylistically similar peers. 
% This allows our framework to harness client heterogeneity, turning heterogeneity into a rich resource for personalization. 

Our main contributions are threefold\footnote{Code will be released upon publication.}
:
\begin{itemize}[leftmargin=1em, itemsep=0.5ex, topsep=0.5ex]
    \item We highlight a key limitation in prior federated TTS frameworks — the high communication cost and the tendency to suppress \textit{stylistic heterogeneity} while preserving speaker timbre.
    \item We propose \textsc{Fed-PISA}, an efficient framework that decouples speaker timbre from collaborative style learning using LoRA and a novel personalized aggregation mechanism.
    \item Experiments on $4$ public datasets demonstrate that \textsc{Fed-PISA} consistently improves style expressivity, speaker similarity,  quality, and communication efficiency over existing baselines.
\end{itemize}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.80\linewidth]{fig1_overview.pdf}
    \caption{An overview of the \textsc{Fed-PISA} framework.}
    \label{fig:fig_overview}
\end{figure*}
% (1) We reveal a core limitation in existing federated TTS methods—the suppression of \textit{stylistic heterogeneity}—and propose \textsc{Fed-PISA}, a framework that decouples identity preservation from collaborative style learning. 

% (2) We design an efficient implementation featuring a decoupled LoRA architecture and personalized aggregation to exploit inter-client heterogeneity. 

% (3) Experiments on multiple benchmarks demonstrate that Fed-PISA consistently improves style expressivity, speaker similarity,  quality, and communication efficiency over existing baselines.
